Task Singular Vectors: Reducing Task Interference in Model Merging

Task Arithmetic has emerged as a simple yet effective method to merge models without additional training. However, by treating entire networks as flat parameter vectors, it overlooks key structural information and is susceptible to task interference. In this paper, we study task vectors at the layer level, focusing on task layer matrices and their singular value decomposition. In particular, we concentrate on the resulting singular vectors, which we refer to as Task Singular Vectors (TSV). Recognizing that layer task matrices are often low-rank, we propose TSV-Compress (TSV-C), a simple procedure that compresses them to 10% of their original size while retaining 99% of accuracy. We further leverage this low-rank space to define a new measure of task interference based on the interaction of singular vectors from different tasks. Building on these findings, we introduce TSV-Merge (TSV-M), a novel model merging approach that combines compression with interference reduction, significantly outperforming existing methods.

==> Z_Cut_pieces/content.tex <==
% It is also interesting to note that our method offers more interpretability with fewer parameters to study. In fact, the second part which starts performing Steps 1, 2, and 3 of the Algorithm \ref{algo}, is obtained thanks to the gained possibility of comparing the fewer selected singular vectors from each task, this leads to the interesting insight that singular vectors from different tasks share some similarity. This is also easily seen in Figure [TODO add ref to the similarity matrix figure], showing intra-task orthogonality with the diagonal structure of the matrix and inter-task interference in the parts of the matrix that compare singular vectors of a task with another task. With steps 1, 2, and 3 we improve the performance of our model merging method by reducing the task interference problem, by approximating the correct transformation from the proper task, and by shifting the weights in this predominant direction.

%%%%%%%%%%%%%%%%%% 
%% CONCLUSIONS
%%%%%%%%%%%%%%%%%%
% In this paper, we have addressed the problem of task interference in model merging. We outlined a connection between task interference and the overlap of singular vectors in task-specific weight by providing a new perspective based on Singular Value Decomposition. Our analysis demonstrated that this overlap is destructive to the performance of merged models. To mitigate this issue, we introduced our new merging approach: Task Singular Vectors.

% TSV reduces task interference by decorrelating singular vectors across different tasks, effectively minimizing their interaction. Through extensive experiments on various computer vision benchmarks, we showed that TSV outperforms existing model merging methods, achieving state-of-the-art results.

% Our contributions offer a new direction for improving model merging by focusing on the geometric properties of Task Vectors. By addressing the possible causes of task interference, our method enhances the performance of merged models without additional training or extra space requirements.

% 

==> cvpr_author_kit/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


